Decentralized Distributed Optimization for Saddle Point Problems

We consider distributed convex-concave saddle point problems over arbitrary connected undirected networks and propose a decentralized distributed algorithm for their solution. The local functions distributed across the nodes are assumed to have global and local groups of variables. For the proposed algorithm we prove non-asymptotic convergence rate estimates with explicit dependence on the network characteristics. To supplement the convergence rate analysis, we propose lower bounds for strongly-convex-strongly-concave and convex-concave saddle-point problems over arbitrary connected undirected networks. We illustrate the considered problem setting by a particular application to distributed calculation of non-regularized Wasserstein barycenters.

==> sections/barycenters_old.tex <==
\section{Applications to the Wasserstein barycenters}\label{sec:wb}

Now we   show the benefits of representing  some convex problems as  convex-concave problems    on the example of the Wasserstein barycenter (WB) problem and demonstrate how it can be solved by Algorithm \ref{alg:mirror_prox_distr}.




Let us suppose that we are given probability measures $q_1, q_2\,..., q_m $ from the probability simplex $\Delta_n$. Then their (fixed-support) WB is a solution of the following  finite-dimensional optimization problem
\begin{equation}\label{eq:W_bary}
   \min_{p \in \Delta_n} \frac{1}{m} \sum_{i=1}^m \mathcal  W(p,q_i),
\end{equation}
where $\mathcal W(p,q) = \min_{X \in  U(p,q)} \langle C, X \rangle$
is  optimal transport  between two histograms $p, q \in \Delta_n$, $C \in \R^{n\times n}_+$ is a given  ground cost matrix, and
$X$ is a transport plan which belongs to the transportation polytope $ U =\{X \in \mathbb R_{+}^{n\times n}, X\boldsymbol{1} = p, X^\top\boldsymbol{1} =q\}$.  As  we consider a general cost matrix $C$, the optimal transport problem  is more general than the problem defining a Wasserstein distance. 

\subsection{Saddle point problem formulation}
Next we reformulate the WB problem \eqref{eq:W_bary} as a saddle point problem (see \cite{dvinskikh2020improved}). To do so, we introduce
  stacked column vector $b_i = (
p^\top, q_i^\top)^\top$,
vectorized cost matrix $d$ of $C$, vectorized transport plan $x \in \Delta_{n^2}$ of $X$,  incidence matrix $A=\{0,1\}^{2n\times n^2}$, vectors $y_i\in [-1,1]^{2n}$ for all $i=1,...,m$. Then Eq. \eqref{eq:W_bary} can be equivalently rewritten as 
\begin{align}\label{eq:def_saddle_prob}
    \min_{ p \in \Delta_n} \frac{1}{m}\sum_{i=1}^m \min_{ x_i\in \Delta_{n^2}} &\max_{~ y_i\in [-1,1]^{2n}}   \{d^\top x_i +2\|d\|_\infty\left(y_i^\top Ax_i -b_i^\top y_i\right)\}.
\end{align}
Clearly, this problem fits the template \eqref{eq:problem_initial}. Finally, we introduce Lagrangian dual variable $\z = (z_1^\top, ..., z^\top_m)^\top \in \Z \triangleq \R^{nm}$, scaled by $\gamma$, to the constraint $\W \p=0$ for the problem \eqref{eq:def_saddle_prob}.  Then we rewrite  the objective in Eq. \eqref{eq:def_saddle_prob}  without normalizing factor $1/m$, thus, we will  minimize this objective with accuracy $m\e$. 
\begin{align}\label{eq:def_saddle_prob2}
         \min_{{ \x \in \X, ~\p \in \Pp } }
         ~\max_{{ \y \in \Y,  ~\z \in \R^{nm} }} 
         &~F(\x,\p,\y, \z)\triangleq   \boldsymbol d^\top \x +2\|d\|_\infty\left(\y^\top\boldsymbol A \x -\b^\top \y \right) +\gamma\la \z,\W\p \ra.
\end{align}
This problem fits the form \eqref{eq:problem_reform} and corresponds to the distributed saddle point formulation of the WB problem. The  gradient operator for $F(\x,\p,\y,\z)$ from Eq. \eqref{eq:def_saddle_prob2} is  defined by
\begin{align*}
    G(\x,\p,\y,\z) = 
    \begin{pmatrix}
  \nabla_\x F(\x,\p,\y,\z) \\
 \nabla_\p F(\x,\p,\y,\z)\\
 -\nabla_\y F(\x,\p,\y,\z) \\
 -\nabla_\z F(\x,\p,\y,\z)\\
    \end{pmatrix} = 
    \begin{pmatrix}
   \boldsymbol d + 2\|d\|_\infty \boldsymbol A^\top \y \\
   \gamma\W^\top\z -   2\|d\|_\infty \{[y_{i}]_{1...n}\}_{i=1}^m \\
  -  2\|d\|_\infty(\A\x - \b)   \\
   -\gamma \W\p
    \end{pmatrix},
\end{align*}
where $[y_{i}]_{1...n}$ is the first $n$ component of vector $y_i\in[-1,1]^{2n}$, and $\{[y_{i}]_{1...n}\}_{i=1}^m$ is a short form of $([y_{1}]_{1...n},[y_{2}]_{1...n},..., [y_{m}]_{1...n})$.


\subsection{Algorithm and convergence rate}
The algorithm proposed in this section is based on the mirror prox algorithm \cite{nemirovski2004prox} on   space $\U \times \V$ which are defined as follows. 
 
\textbf{Setup.} 
     We endow space $\V \triangleq \Y \times \Z  \triangleq [-1,1]^{2nm} \times \R^{nm}$  with the standard Euclidean setup:  
 \begin{itemize}
     \item the Euclidean norm $ \|\cdot\|_2$
     \item prox-function $d_\v(\v) = \frac{1}{2}\|\v\|_2^2$
     \item the corresponding Bregman divergence 
 $B_{\v} = \frac{1}{2}\|\v -\breve \v\|_2^2$
 \end{itemize}
 We also define  $R^2_\v = \max_{\v \in \V \cap B_R(0) }d_\v(\v) - \min_{\v \in \V \cap B_R(0)}d_\v(\v)$. Here $B_R(0)$ is a ball of radius $R$ centered in $0$.
     We endow space  $\U \triangleq \X\times \Pp \triangleq \prod^m \Delta_{n^2} \times \prod^m \Delta_{n}  $ with 
     \begin{itemize}
         \item  norm $ \|\u\|_\u = \sqrt{\sum_{i=1}^m \|x_i\|^2_1 +\sum_{i=1}^m\|p_i\|_1^2}$, where $\|\cdot\|_1 $ is the $\ell_1$-norm
         \item  prox-function
$d_\u(\u) = \sum_{i=1}^m  \la x_i,\log x_i \ra +\sum_{i=1}^m \la p_i,\log p_i \ra$
         \item the  corresponding  Bregman divergence
\begin{align*}
B_\u(\u, \breve \u) &= \textstyle \sum_{i=1}^m  \langle x_i, \log (x_i /  \breve x_i) \rangle -\sum_{i=1}^m\boldsymbol 1_{n^2}^\top( x_i -  \breve x_i) + \sum_{i=1}^m  \langle p_i, \log (p_i /  \breve p_i) \rangle \\
&-\textstyle \sum_{i=1}^m\boldsymbol 1_{n}^\top( p_i -  \breve p_i)
\end{align*}
     \end{itemize}
We also define $R^2_\u = \max_{\u \in  \U }d_\u(\u) - \min_{\u \in  \U }d_\u(\u)$.

Finally, we endow the space $\U \times \V$ with
\begin{itemize}
    \item prox-function $ a d_\u(\u)+ b d_\v(\v)$, where   $a = \nicefrac{1}{R_{\u}^2}$, $b =\nicefrac{1}{R_{\v}^2} $
    \item the corresponding Bregman divergence  $a B_{\u}(\u, \breve \u) + b B_\v(\v,\breve \v)$, where   $a = \nicefrac{1}{R_{\u}^2}$, $b =\nicefrac{1}{R_{\v}^2} $
\end{itemize}








\begin{lemma}\label{lm:Lipsch1}
Objective $F(\u,\v)$ in \eqref{eq:def_saddle_prob2} is $ (L_{\u\u},L_{\u\v}, L_{\v\u}, L_{\v\v})$-smooth with $L_{\u\u}=L_{\v\v}=0$ and $L_{\u\v}=L_{\v\u} = \sqrt{{8\|d\|^2_\infty}+ \gamma^2\lm_{\max} (W)^2} $.
\end{lemma}







The proof of this lemma is given in the Appendix \ref{app:application_of_mirror_prox}. This lemma   allows us to obtain the following convergence result
\begin{theorem}\label{Th:first_alg11}
Let $\gamma ={\sqrt{8}\|d\|_\infty}/{\lm_{\max}(W)} $, $\|\z\|^2_2 \leq R^2\leq \sqrt{2}mn\|d\|_\infty\chi$. Then $R_{\u}=\sqrt{3m\log n}$, $R_\v = \sqrt{2mn\|d\|_\infty\chi}$
and after $ N =  {16\|d\|_\infty\sqrt{6n\log n \|d\|_\infty \chi}}/{\e}$ iterations  Algorithm \ref{MP_WB_distr}   with 
$\eta  = \frac{1}{8m\|d\|_\infty\sqrt{6n\log n \|d\|_\infty \chi}}$
outputs a pair $(\widetilde \u, \widetilde \v)$ such that
\begin{align*}
    \max_{{ \y \in \Y,~ \|\z\|_2 \leq R }} \frac{1}{m}F\left( \widetilde \u, \y,\z\right) - \min_{ { \x \in \X,~ \p \in \Pp }} \frac{1}{m} F\left(\x,\p,\widetilde \v\right)  \leq \e.
\end{align*}
The total complexity of Algorithm \ref{MP_WB_distr} per node is 
\[O\left(\frac{n^2}{\e}\sqrt{n\log n} \sqrt{\chi}
    \|d\|_\infty^{3/2}  \right).\]
\end{theorem}
The proof of this theorem is in the Appendix \ref{app:Th_WB}.

For the star network, we can compare the complexity of Mirror-Prox per node with the per node  complexity  of the IBP, that is $ \widetilde O\left({ n^2 
}/{\e^2}\right)$  \cite{kroshnin2019complexity}, or with the per node complexity of the FastIBP , that is $ \widetilde O\left({n^{7/3}}/{{\e^{7/3}}}\right)$ \cite{lin2020fixed}. Distributed Mirror-Prox has better dependence on $\e$, namely $1/\e$, as well as the  accelerated IBP \cite{guminov2019accelerated} and primal-distributed algorithm from \cite{kroshnin2019complexity} with $\widetilde O\left({n^2 \sqrt{n}}/{\e}\right)$ complexities per node.  However, all of these regularization-based method have  a strong limitation regarding the regularization parameter: numerical instability at small regularization parameter. This is the case when a high precision is desired (as the regularization parameter  must be chosen proportionally to $\e$).


==> sections/sliding.tex <==
\begin{lemma}
	Iterates of Algorithm~\ref{alg:sliding} satisfy the following inequality:
	\begin{align}
		\sqn{\zeta^{k+1} - \zeta^*}
		&\leq (1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}+ \left(3\eta\mu_g + \eta^2L_A^2 -  1\right)\sqn{\zeta^k - \theta^k} \notag \\
		&\quad+ \left(\frac{4}{\eta\mu_g} + \frac{4\eta L_B^2}{\mu_g}\right) \sqn{\theta^k - \hat{\theta}^k}. \label{sliding:eq:1}
	\end{align}
\end{lemma}
\begin{proof}
    % could not fix troubles with algorithm line cross reference
    % doing it manually
    % sliding:line:z -> 2
    % sliding:line:y -> 3
    % sliding:line:w -> 4
    % sliding:line:x -> 5
	We start with using line 5 %\ref{sliding:line:x} 
	of Algorithm~\ref{alg:sliding}:
	\begin{align*}
		\sqn{\zeta^{k+1} - \zeta^*}
		&=
		\sqn{\proj_Q(\omega^k) - \proj_Q(\zeta^*)}
		\\&\leq
		\sqn{\omega^k - \zeta^*}.
		\\&=
		\sqn{\zeta^k - \zeta^*} + 2\<\omega^k - \zeta^k, \zeta^k - \zeta^*> + \sqn{\omega^k - \zeta^k}
		\\&=
		\sqn{\zeta^k - \zeta^*} + 2\<\omega^k - \zeta^k, \theta^k - \zeta^*>  + 2\<\omega^k - \zeta^k,\zeta^k - \theta^k> + \sqn{\omega^k - \zeta^k}
		\\&=
		\sqn{\zeta^k - \zeta^*} + 2\<\omega^k - \zeta^k, \theta^k - \zeta^*>  + \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}.
	\end{align*}
	Using line 4 %\ref{sliding:line:w}
	of Algorithm~\ref{alg:sliding} we get
	\begin{align*}
		\sqn{\zeta^{k+1} - \zeta^*}
		&\leq
		\sqn{\zeta^k - \zeta^*} + 2\<\theta^k + \eta(A(\zeta^k) - A(\theta^k)) - \zeta^k, \theta^k - \zeta^*> \\
		&\quad+ \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k} \\
		&= \sqn{\zeta^k - \zeta^*} + 2\<\theta^k + \eta A(\zeta^k) - \zeta^k, \theta^k - \zeta^*>-2\eta\<A(\theta^k), \theta^k - \zeta^*> \\
		&\quad+ \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\end{align*}
	Using line 2 %\ref{sliding:line:z}
	of Algorithm~\ref{alg:sliding} we get
	\begin{align*}
	\sqn{\zeta^{k+1} - \zeta^*}
	&\leq
	\sqn{\zeta^k - \zeta^*} + 2\<\theta^k - \nu^k, \theta^k - \zeta^*>  - 2\eta\<A(\theta^k), \theta^k - \zeta^*> + \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\\&=
	\sqn{\zeta^k - \zeta^*} - 2\<\hat{\theta}^k - \nu^k, \zeta^* - \theta^k>  - 2\eta\<A(\theta^k), \theta^k - \zeta^*> + \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\\&\quad+
	2\<\theta^k - \hat{\theta}^k,\theta^k - \zeta^*>.
	\end{align*}
	Using \eqref{sliding:eq:prox} we get
	\begin{align*}
	\sqn{\zeta^{k+1} - \zeta^*}
	&\leq
	\sqn{\zeta^k - \zeta^*} + 2\eta\<B(\hat{\theta}^k), \zeta^* - \theta^k>  - 2\eta\<A(\theta^k), \theta^k - \zeta^*> + \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\\&\quad+
	2\<\theta^k - \hat{\theta}^k,\theta^k - \zeta^*>
	\\&=
	\sqn{\zeta^k - \zeta^*} - 2\eta\<B(\theta^k), \theta^k - \zeta^* >  - 2\eta\<A(\theta^k), \theta^k - \zeta^*> + \sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\\&\quad+
	2\<\theta^k - \hat{\theta}^k + \eta (B(\theta^k) - B(\hat{\theta}^k)),\theta^k - \zeta^*>.
	\end{align*}
	Using that $g(\zeta) = A(\zeta) + B(\zeta)$ and $\mu_g$-strong monotonicity of $g$ we get
	\begin{align*}
		\sqn{\zeta^{k+1} - \zeta^*}
		&\leq
		\sqn{\zeta^k - \zeta^*} - 2\eta\<g(\theta^k), \theta^k - \zeta^* >  +\sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
		\\&\quad+
		2\<\theta^k - \hat{\theta}^k + \eta (B(\theta^k) - B(\hat{\theta}^k)),\theta^k - \zeta^*>
		\\&\leq
		\sqn{\zeta^k - \zeta^*}- 2\eta\mu_g\sqn{\theta^k - \zeta^*} - 2\eta\<g(\zeta^*), \theta^k - \zeta^* >  +\sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
		\\&\quad+
		2\<\theta^k - \hat{\theta}^k + \eta (B(\theta^k) - B(\hat{\theta}^k)),\theta^k - \zeta^*>.
	\end{align*}
	By definition of $\zeta^*$ and Young's inequality we get
	\begin{align*}
		\sqn{\zeta^{k+1} - \zeta^*}
		&\leq
		\sqn{\zeta^k - \zeta^*}- 2\eta\mu_g\sqn{\theta^k - \zeta^*}+\sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
		\\&\quad+
		2\<\theta^k - \hat{\theta}^k + \eta (B(\theta^k) - B(\hat{\theta}^k)),\theta^k - \zeta^*>
		\\&\leq
		\sqn{\zeta^k - \zeta^*}- 2\eta\mu_g\sqn{\theta^k - \zeta^*}+\sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
		\\&\quad+
		\frac{\eta\mu_g}{2}\sqn{\theta^k - \zeta^*} + \frac{2}{\eta\mu_g}\sqn{\theta^k - \hat{\theta}^k + \eta (B(\theta^k) - B(\hat{\theta}^k))}
		\\&\leq
		\sqn{\zeta^k - \zeta^*}- \frac{3\eta\mu_g}{2}\sqn{\theta^k - \zeta^*}+\sqn{\omega^k - \theta^k} - \sqn{\zeta^k - \theta^k}
		\\&\quad+
		\frac{4}{\eta\mu_g}\sqn{\theta^k - \hat{\theta}^k} + \frac{4\eta}{\mu_g}\sqn{B(\theta^k) - B(\hat{\theta}^k)}.
	\end{align*}
	Using line 4 %\ref{sliding:line:w}
	of Algorithm~\ref{alg:sliding} we get
	\begin{align*}
		\sqn{\zeta^{k+1} - \zeta^*}
		&\leq
		\sqn{\zeta^k - \zeta^*}- \frac{3\eta\mu_g}{2}\sqn{\theta^k - \zeta^*}+ \eta^2\sqn{A(\zeta^k) - A(\theta^k)} - \sqn{\zeta^k - \theta^k}
		\\&\quad+
		\frac{4}{\eta\mu_g}\sqn{\theta^k - \hat{\theta}^k} + \frac{4\eta}{\mu_g}\sqn{B(\theta^k) - B(\hat{\theta}^k)}.
	\end{align*}
	Using \eqref{eq:LA} and \eqref{eq:LB} we get
	\begin{align*}
	\sqn{\zeta^{k+1} - \zeta^*}
	&\leq
	\sqn{\zeta^k - \zeta^*}- \frac{3\eta\mu_g}{2}\sqn{\theta^k - \zeta^*}+ \eta^2L_A^2\sqn{\zeta^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\\&\quad+
	\frac{4}{\eta\mu_g}\sqn{\theta^k - \hat{\theta}^k} + \frac{4\eta L_B^2}{\mu_g}\sqn{\theta^k - \hat{\theta}^k}.
	\end{align*}
	Using inequality $\sqn{a+b} \geq \frac{2}{3}\sqn{a} - 2\sqn{b}$ we get
	\begin{align*}
	\sqn{\zeta^{k+1} - \zeta^*}
	&\leq
	\sqn{\zeta^k - \zeta^*}- \frac{3\eta\mu_g}{2}\left[\frac{2}{3}\sqn{\zeta^k - \zeta^*} - 2\sqn{\zeta^k - \theta^k}\right]+ \eta^2L_A^2\sqn{\zeta^k - \theta^k} 
	\\&\quad- \sqn{\zeta^k - \theta^k}+
	\frac{4}{\eta\mu_g}\sqn{\theta^k - \hat{\theta}^k} + \frac{4\eta L_B^2}{\mu_g}\sqn{\theta^k - \hat{\theta}^k}
	\\&\leq
	(1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}+ 3\eta\mu_g\sqn{\zeta^k - \theta^k} + \eta^2L_A^2\sqn{\zeta^k - \theta^k} - \sqn{\zeta^k - \theta^k}
	\\&\quad+
	\frac{4}{\eta\mu_g}\sqn{\theta^k - \hat{\theta}^k} + \frac{4\eta L_B^2}{\mu_g}\sqn{\theta^k - \hat{\theta}^k}
	\\&=
	(1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}+ \left(3\eta\mu_g + \eta^2L_A^2 -  1\right)\sqn{\zeta^k - \theta^k}
	\\&\quad+ 
	\left(\frac{4}{\eta\mu_g} + \frac{4\eta L_B^2}{\mu_g}\right) \sqn{\theta^k - \hat{\theta}^k}.
	\end{align*}
\end{proof}


\begin{lemma}
	Let $\theta^k$ be the output of Forward-Backward-Forward algorithm for solving auxiliary problem \eqref{sliding:eq:prox} after $T$ iterations starting at point $\zeta^k$. Choosing $\delta \in (0, 1/4]$ and number of iterations
	\begin{equation}\label{sliding:eq:T}
		T = \cO \left( \left(1 + \eta L_B\right) \log \frac{1}{\delta}\right)
	\end{equation}
	implies
	\begin{equation}\label{sliding:eq:2}
		\sqn{\hat{\theta}^k - \theta^k} \leq 4\delta\sqn{\zeta^k - \theta^k}.
	\end{equation}
\end{lemma}
\begin{proof}
	Problem \eqref{sliding:eq:prox} is a variational inequality of the form
	\begin{equation*}
		\<\hat{B}^k(\hat{\theta}^k), \zeta - \hat{\theta}^k> \geq 0 \text{ for all } \zeta \in Q,
	\end{equation*}
	where operator $\hat{B}^k \colon Q \rightarrow \R^d$ is defined in the following way
	\begin{equation*}
		\hat{B}^k(\zeta) = \eta B(\zeta) + \zeta - \nu^k.
	\end{equation*}
	Operator $\hat{B}^k(\zeta)$ is 1-strongly monotone and $(1 + \eta L_B)$-Lipschitz. Hence, applying the standard result on Forward-Backward-Forward algorithm implies
	\begin{equation*}
		\sqn{\theta^k - \hat{\theta}^k} \leq \delta\sqn{\zeta^k - \hat{\theta}^k}.
	\end{equation*}
	Moreover,
	\begin{align*}
		\sqn{\theta^k - \hat{\theta}^k} &\leq \delta\sqn{\zeta^k - \hat{\theta}^k}
		\\&\leq
		2\delta\sqn{\zeta^k - \theta^k} + 2\delta\sqn{\theta^k - \hat{\theta}^k}
		\\&\leq
		2\delta\sqn{\zeta^k - \theta^k} + \frac{1}{2}\sqn{\theta^k - \hat{\theta}^k},
	\end{align*}
	where the last inequality follows from $\delta \leq \frac{1}{4}$. Rearranging gives \eqref{sliding:eq:2}.
\end{proof}

\begin{lemma}
 Apply Algorithm~\ref{alg:sliding} to the problem \eqref{eq:problem_reform}. On each iteration of Algorithm~\ref{alg:sliding} solve auxiliary problem \eqref{sliding:eq:prox} on line 3 %\ref{sliding:line:y}
 with $T$ iterations of Forward-Backward-Forward algorithm starting at point $\zeta^k$, where $T$ is given by \eqref{sliding:eq:T}
 Choosing $\delta$ to be
 \begin{equation}\label{sliding:delta}
 	\delta = \min\left\{\frac{1}{4}, \left[\frac{64}{\eta\mu_g} + \frac{64\eta L_B^2}{\mu_g}\right]^{-1}\right\},
 \end{equation}
 choosing stepsize $\eta$ to be
 \begin{equation}\label{sliding:eta}
 	\eta = \min\left\{\frac{1}{2L_A}, \frac{1}{6\mu_g}\right\}
 \end{equation}
 and choosing number of iterations $N$ to be
 \begin{equation}\label{sliding:K}
 	N = \frac{1}{\eta\mu_g} \log \frac{\sqn{\zeta^0 - \zeta^*}}{\epsilon}
 \end{equation}
 implies
 \begin{equation}\label{sliding:eq:3}
 	\sqn{\zeta^N - \zeta^*} \leq \epsilon.
 \end{equation}
\end{lemma}
\begin{proof}
	Using \eqref{sliding:eq:1} together with \eqref{sliding:eq:2}, we get
	\begin{align*}
		\sqn{\zeta^{k+1} - \zeta^*}
		&\leq (1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}+ \left(3\eta\mu_g + \eta^2L_A^2 -  1\right)\sqn{\zeta^k - \theta^k}
		\\
		&\quad+ 4\delta\left(\frac{4}{\eta\mu_g} + \frac{4\eta L_B^2}{\mu_g}\right) \sqn{\zeta^k - \theta^k}.
	\end{align*}
	Plugging $\delta$ defined by \eqref{sliding:delta} gives
	\begin{align*}
	\sqn{\zeta^{k+1} - \zeta^*}&\leq (1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}+ \left(3\eta\mu_g + \eta^2L_A^2 -  1\right)\sqn{\zeta^k - \theta^k}
	+
	\frac{1}{4}\sqn{\zeta^k - \theta^k}
	\\&=
	(1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}+ \left(3\eta\mu_g + \eta^2L_A^2 -  \frac{3}{4}\right)\sqn{\zeta^k - \theta^k}.
	\end{align*}
	Plugging $\eta$ defined by \eqref{sliding:eta} gives
	\begin{align*}
	\sqn{\zeta^{k+1} - \zeta^*}\leq
	(1-\eta\mu_g)\sqn{\zeta^k - \zeta^*}.
	\end{align*}
	After telescoping and using $N$ defined by $\eqref{sliding:K}$ we get \eqref{sliding:eq:3}, which concludes the proof.
\end{proof}

\begin{corollary}
	Without loss of generality assume $L_A \leq L_B$. Total number of computations of $A(\zeta)$ is
	\begin{equation*}
		N_A = N = \cO\left(\left(1 + \frac{L_A}{\mu_g}\right)\log \frac{\sqn{\zeta^0 - \zeta^*}}{\epsilon}\right).
	\end{equation*}
	Total number of computations of $B(\zeta)$ is
	\begin{align*}
		N_B &= N \times T= \cO\left(\left(1 + \min\left\{\frac{1}{\mu_g}, \frac{1}{L_A}\right\}L_B\right)\left(1 + \frac{L_A}{\mu_g}\right)\log\frac{1}{\delta}\log \frac{\sqn{\zeta^0 - \zeta^*}}{\epsilon}\right)
		\\&=
		\cO\left(\left(
		1 + \min\left\{\frac{L_B}{\mu_g}, \frac{L_B}{L_A}\right\} + \frac{L_A}{\mu_g} + \min\left\{\frac{L_BL_A}{\mu_g^2}, \frac{L_B}{\mu_g}\right\}
		\right)\log\frac{1}{\delta}\log \frac{\sqn{\zeta^0 - \zeta^*}}{\epsilon}\right)
		\\&\leq
		\cO\left(\left(
		1 + \frac{L_A}{\mu_g}+ \frac{L_B}{\mu_g}
		\right)\log\frac{1}{\delta}\log \frac{\sqn{\zeta^0 - \zeta^*}}{\epsilon}\right)
		\\&\leq
		\cO\left(\left(
		1 +\frac{L_B}{\mu_g}
		\right)\log\frac{1}{\delta}\log \frac{\sqn{\zeta^0 - \zeta^*}}{\epsilon}\right).
	\end{align*}
\end{corollary}


==> sections/tmp_denotations.tex <==
{\color{red}
\section{DENOTATIONS}

Number of nodes: m

Initial function: $f(x, y) = \frac{1}{m}\sum_{i=1}^m f_i(x, y)$

Inflated function: $F(\bx, \by) = \sum_{i=1}^m f_i(x_i, y_i)$

Dual variables: $\bz$ corresponding to $\bx$, $\bt$ corresponding to $\by$. I.e. 
$$
\min_{\bx, \bt}~ F(\bx, \by) + \gamma_x\angles{\bz, \mWx\bx} + \gamma_y\angles{\bs, \mWy\by}
$$

Minimization variables: $\bu = (\bx^\top, \bs^\top)^\top$. Maximization variables: $\bv = (\by^\top ,\bz^\top)^\top$.

Additional local variables: $\bp$ (min), $\bq$ (max).

Sets: $\sX, \sY, \sZ, \sS, \sU, \sV$.
}
